Intelligent Control in 6G Open RAN: Security Risk or Opportunity?

The Open Radio Access Network (Open RAN) framework, emerging as the cornerstone for Artificial Intelligence (AI)-enabled Sixth-Generation (6G) mobile networks, heralds a transformative shift in radio access network architecture. As the adoption of Open RAN accelerates, ensuring its security becomes critical. The RAN Intelligent Controller (RIC) plays a central role in Open RAN by improving network efficiency and flexibility. Nevertheless, it also brings about potential security risks that need careful scrutiny. Therefore, it is imperative to evaluate the current state of RIC security comprehensively. This assessment is essential to gain a profound understanding of the security considerations associated with RIC. This survey combines a comprehensive analysis of RAN security, tracing its evolution from 2G to 5G, with an in-depth exploration of RIC security, marking the first comprehensive examination of its kind in the literature. Real-world security incidents involving RIC are vividly illustrated, providing practical insights. The study evaluates the security implications of the RIC within the 6G Open RAN context, addressing security vulnerabilities, mitigation strategies, and potential enhancements. It aims to guide stakeholders in the telecom industry toward a secure and dependable telecommunications infrastructure. The article serves as a valuable reference, shedding light on the RIC's crucial role within the broader network infrastructure and emphasizing security's paramount importance. This survey also explores the promising security opportunities that the RIC presents for enhancing network security and resilience in the context of 6G mobile networks. It outlines open issues, lessons learned, and future research directions in the domain of intelligent control in 6G open RAN, facilitating a comprehensive understanding of this dynamic landscape.

==> table.tex <==
\setlist{leftmargin=*}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
%\renewcommand{\arraystretch}{0.5}
\begin{table*}[htbp]
	\caption{Summary of Important Surveys Related to RIC Security} \label{tbl:ProsAndCons}
    \centering
% 	\footnotesize

	\begin{tabular}{|m{1.3cm}|m{0.5cm}|m{0.5cm}|m{4.5cm}|m{4.2cm}|m{4.2cm}|}
		\hline
		\textbf{Aspect} 
		%&\textbf{Research Type} 
		&\textbf{Year} 
		&\textbf{Ref.} 
		&\textbf{Main contributions} 
		&\textbf{Relevance to our survey (advantages)}
		&\textbf{Disadvantages (Shortcomings)}
		\\\hline
		\multirow{3}{*}{\begin{tabular}{@{}c@{}}Open RAN\\General\end{tabular}} 
		&2023  
        & ~\cite{polese2023understanding}
        & \begin{itemize}
             \item Comprehensive survey on O-RAN architecture, interfaces \& its innovations
             \item Discussing challenges in O-RAN
             \item Discussing AI and ML in O-RAN
         \end{itemize} 
         
        &  \begin{itemize}
             \item Discussed the new security challenges in O-RAN
             \item Discussed the new security opportunities in O-RAN
         \end{itemize}  &  
         
        \begin{itemize}
             \item  lack of specific emphasis on security risks in RIC
             \item The omission of addressing the unique security solutions in RIC
             
         \end{itemize} 
         \\\cline{2-6} 
		& 2022 
		& ~\cite{abdalla2022toward}
		& 
		\begin{itemize}
             \item A survey on O-RAN architecture, components and interfaces
             \item evaluating O-RAN capabilities in various use cases

         \end{itemize}
		&  \begin{itemize}
             \item A section on security issues in O-RAN with a focus on specifications.
             \item Highlighting RIC functionalities
             
         \end{itemize} & 
         \begin{itemize}
             \item  lack of specific emphasis on security risks in RIC
             \item The omission of addressing the unique security solutions in RIC
             \item Limited Bibliography

         \end{itemize} \\\cline{2-6}
	        & 2023 
		& ~\cite{zhao2022survey}
		&\begin{itemize}
             \item An overview of open-source wireless networks including O-RAN
             \item  Focuses on various frameworks \& significant technologies in the area of O-RAN
             
         \end{itemize} 
		&  \begin{itemize}
             \item An up-to-date analysis of various types of security risks in O-RAN
             \item Examining security risks in SDN
             
         \end{itemize} 
         
         & 
         \begin{itemize}
         \item No specific emphasis on the security risks in RIC
         \item No explicit emphasis on the security solutions in RIC

         \end{itemize} 
         \\\hline
         
		\multirow{3}{*}{\begin{tabular}{@{}c@{}}Open RAN\\Security\end{tabular}}
		& 2022 
		& ~\cite{mimran2022evaluating}
		& \begin{itemize}
             \item A survey \& threat analysis on O-RAN architecture
             \item Evaluating the possibility of past attacks in different domains within O-RAN

         \end{itemize} 
		& \begin{itemize}
             \item Minor consideration for Open RAN centralized control plane vulnerabilities.
             \item Considering the entire O-RAN security aspects with no deep focus
             
         \end{itemize} 
         
         &  \begin{itemize}
             \item Missing industrial use cases
             \item Missing Examples of real-world attacks
             \item No explicit focus on security threats \& solutions in RIC
         \end{itemize} 
	        \\\cline{2-6}
        &2022  
        & ~\cite{liyanage2022open}
        & 	\begin{itemize}
             \item A comprehensive survey on the security threats in O-RAN architecture
             \item Discussing potential security solutions \& benefits of O-RAN

         \end{itemize} 
        &  \begin{itemize}
             \item Focus on generic Open RAN threats and solutions based on Open RAN SFG works
             \item Classifying security-related risks, and Present Open RAN specific security solutions
             
         \end{itemize} & \begin{itemize}
         \item No specific emphasis on the security risks in RIC
         \item No explicit emphasis on the security solutions in RIC
         
         \end{itemize}  \\\cline{2-6}
        & 2020 
        & ~\cite{boswell2020security} 
        & \begin{itemize}
             \item Overview of the security challenges in Open RAN architecture for industrial use cases
             
         \end{itemize} 
        &   \begin{itemize}
             \item White paper on O-RAN security
             
             
         \end{itemize} 
         & \begin{itemize}
             \item limited bibliographic survey
             \item White paper on O-RAN security
         \end{itemize} 
         \\\hline
        \multirow{2}{*}{\begin{tabular}{@{}c@{}}5G RAN\\Security\end{tabular}} 
		 &2019&~\cite{habibi2019comprehensive}&  
		 \begin{itemize}
             \item An examination and comparison of different RAN structures applicable to 5G
             \item An exploration of the fundamental technologies enabling the 5G RAN
 
         \end{itemize} &
		   \begin{itemize}
             \item Focus on threat analysis specific to the 5G RAN
             \item addressing existing challenges and future works related to 5G RAN

         \end{itemize} & \begin{itemize}
             \item No focus on O-RAN security
             \item No focus on RIC security
            
         \end{itemize} 

		 \\\cline{2-6}
		 &2017&~\cite{tian2017survey}&  \begin{itemize}
             \item Examining the security of 5G C-RAN
             \item  Analyzing security measures in wireless netwroks, SDRs \& CRNs
             \item  Identifying security risks in C-RAN
             \item Suggesting security/trust criteria
         \end{itemize} &
		   \begin{itemize}
             \item Focus on threat analysis specific to the 5G C-RAN
             \item  Introducing trust and security necessities in C-RAN
             
         \end{itemize} & 
         \begin{itemize}
             \item No focus on security challenges in O-RAN
             \item No focus on RIC security
             
         \end{itemize} 

		 \\
		 \hline
		 \multirow{2}{*}{\begin{tabular}{@{}c@{}}SDN\\Security\end{tabular}}
		 &2016&~\cite{khan2016topology}&
		\begin{itemize}
             \item A comprehensive tutorial and survey on vulnerabilities of control plane in SDN
             \item Discussion on topology discovery attacks
             
         \end{itemize} &
	   \begin{itemize}
             \item Security concerns were discussed regarding a centralized control system
             \item Solutions were discussed in a SDN controller
             
         \end{itemize} & \begin{itemize}
             \item No focus on O-RAN
             \item No focus on RIC
         \end{itemize} 
	    \\\cline{2-6}
	    		 &2018&~\cite{abdou2018comparative}&
	        \begin{itemize}
             \item Describing control functions in SDN
             \item  Examines the risks and defense in SDN
             \item Presenting a framework for comparison of the security using two threat models
         \end{itemize} &
	   \begin{itemize}
             \item The discussion focused on security concerns related to a centralized control system
             \item Various solutions were explored to address the security issues associated with a centralized control system

         \end{itemize} & \begin{itemize}
             
             \item  lack of specific emphasis on security risks in RIC
             \item The omission of addressing the unique security solutions in RIC
         \end{itemize} 
	    \\\hline
	    
	\end{tabular}

\end{table*}



\begin{table*}[htbp]
    \caption{Resilient RIC Security Measures and Vulnerabilities Mitigated. $\LEFTcircle$: Partial Discussion (i.e. At least one specialized section is presented but lacks a thorough examination). $\Circle$: Not Supported}
    \label{tbl:RICSecurityFeaturesReversed}
    \centering
    \scriptsize
    \begin{tabular}{m{5cm}m{10cm}*{7}{>{\centering\arraybackslash}m{0.25cm}}}
         \hline
         \rule{0pt}{2ex}
        \textbf{RIC Security Controls} & \textbf{Technical Details} &  \textbf{V-01} & \textbf{V-02} & \textbf{V-03} & \textbf{V-04} & \textbf{V-05} & \textbf{V-06} &\textbf{V-07} \\
        \hline
        Ensuring secure \textit{xApp} deployment & Verify digital signatures, use TLS for secure communication, and OAuth 2.0 for registration & $\Circle$ & $\Circle$ & $\Circle$ & $\Circle$ & $\Circle$ & $\Circle$ & $\Circle$  \\
        Ensuring strict API access controls & Employ mutual authentication (mTLS or IPsec) and OAuth 2.0 for authorization & $\Circle$ & $\Circle$ & $\Circle$ & $\Circle$ & $\Circle$ & $\Circle$ & $\Circle$ \\
        Ensuring granular access control for R/UE-NIB & Implement RBAC using database tokens and Security Function validation & $\LEFTcircle$ & $\LEFTcircle$ & $\CIRCLE$ & $\LEFTcircle$ & $\Circle$& $\Circle$& $\Circle$  \\
        Ensuring Secure Software Development & Following secure software development practices and monitoring for vulnerabilities and patches & $\CIRCLE$ & $\CIRCLE$ & $\LEFTcircle$ & $\Circle$ & $\LEFTcircle$ & $\Circle$ & $\Circle$  \\
        Ensuring Secure RIC Interface Communications & Use IPsec, DTLS, and TLS with mutual authentication for different RIC interfaces & $\Circle$ & $\LEFTcircle$ & $\CIRCLE$ & $\Circle$ & $\Circle$ & $\Circle$& $\Circle$  \\
        Protecting Against Conflicting xApps & Using the Conflict Mitigation function with guidance during xApp Registration
 & $\CIRCLE$ & $\LEFTcircle$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\LEFTcircle$ & $\Circle$ \\
        \hline
    \end{tabular}
\end{table*}

\begin{table*}[htbp]
    \caption{Resilient RIC Security Measures and Vulnerabilities Mitigated$\CIRCLE$: Mitigated. $\LEFTcircle$: Partial Mitegated. $\Circle$: Not Mitigated}
    \label{tbl:RICSecurityFeaturesReversed}
    \centering
    \scriptsize
    \begin{tabular}{m{5.5cm}m{9.8cm}*{7}{>{\centering\arraybackslash}m{0.23cm}}}
         \hline
         %\rule{0pt}{3ex}
        \textbf{RIC Security Controls} & \textbf{Technical Details} &  \textbf{V-01} & \textbf{V-02} & \textbf{V-03} & \textbf{V-04} & \textbf{V-05} & \textbf{V-06} &\textbf{V-07} \\
        \hline
        Ensuring secure \textit{xApp} deployment & \begin{itemize}[leftmargin=*,nosep] \vspace{1mm}
            \item Digital signature generation and validation.
            \item Secure TLS communication during provisioning.
            \item Authentication in onboarding, provisioning, and registration.\vspace{-2mm}
        \end{itemize} & $\Circle$ & $\Circle$ & $\Circle$ & $\Circle$ & $\Circle$ & $\Circle$ & $\Circle$  \\\hline
        Ensuring strict API access controls & \begin{itemize}[leftmargin=*,nosep]\vspace{1mm}
            \item Mutual authentication (mutual TLS or IPsec).
            \item Utilization of OAuth 2.0 for authorization.\vspace{-2mm}
        \end{itemize} & $\Circle$ & $\Circle$ & $\Circle$ & $\Circle$ & $\Circle$ & $\Circle$ & $\Circle$ \\\hline
        Ensuring granular access control for R/UE-NIB & \begin{itemize}[leftmargin=*,nosep]\vspace{1mm}
            \item Role-Based Access Control (RBAC).
            \item Database token generation and validation.\vspace{-2mm}
        \end{itemize} & $\LEFTcircle$ & $\LEFTcircle$ & $\CIRCLE$ & $\LEFTcircle$ & $\Circle$& $\Circle$& $\Circle$  \\\hline
        Ensuring secure software development & \begin{itemize}[leftmargin=*,nosep]\vspace{1mm}
            \item Maintain an inventory of open-source components and track vulnerabilities.
            \item Continuous monitoring for new risks and vulnerabilities.\vspace{-2mm}
        \end{itemize} & $\CIRCLE$ & $\CIRCLE$ & $\LEFTcircle$ & $\Circle$ & $\LEFTcircle$ & $\Circle$ & $\Circle$  \\\hline
        Ensuring secure RIC interface communications & \begin{itemize}[leftmargin=*,nosep]\vspace{1mm}
            \item Utilize secure protocols like IPsec, TLS, and DTLS for data confidentiality and integrity.
            \item Safeguard against eavesdropping and unauthorized O\&M connectivity.\vspace{-2mm}
        \end{itemize} & $\Circle$ & $\LEFTcircle$ & $\CIRCLE$ & $\Circle$ & $\Circle$ & $\Circle$& $\Circle$  \\\hline
        Protecting against conflicting \textit{xApps} & \begin{itemize}[leftmargin=*,nosep]\vspace{1mm}
            \item Function initiated by authorized xApps, Subscription Management, or the function itself.\vspace{-2mm}
        \end{itemize} & $\CIRCLE$ & $\LEFTcircle$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\LEFTcircle$ & $\Circle$ \\
        \hline
    \end{tabular}
\end{table*}
